Ensembler: Protect Collaborative Inference Privacy from Model Inversion Attack via Selective Ensemble

For collaborative inference through a cloud computing platform, it is sometimes essential for the client to shield its sensitive information from the cloud provider. In this paper, we introduce Ensembler, an extensible framework designed to substantially increase the difficulty of conducting model inversion attacks by adversarial parties. Ensembler leverages selective model ensemble on the adversarial server to obfuscate the reconstruction of the client's private information. Our experiments demonstrate that Ensembler can effectively shield input images from reconstruction attacks, even when the client only retains one layer of the network locally. Ensembler significantly outperforms baseline methods by up to 43.5% in structural similarity while only incurring 4.8% time overhead during inference.

==> content/3_analysis.tex <==
\section{Analysis on Splitting Between Client and Server}

Previous work from \cite{He2019} provided a systematic analysis on the recovery difficulty and quality of the above mentioned model-inversion attack. Their work analyzed effects on reconstruction quality from loosening assumptions of auxiliary information available to the server (DNN architecture and training dataset), as well as choosing different split points (h) between the client and the server. However, their work was based on a simple 6-layer convolutional neural network (CNN), which is seldom used in today's service. In this section, we further their analysis upon more practical architectures, namely ResNet-18 and VGG-16.




\begin{figure}{}
    \centering
    \includegraphics[scale=0.35]{img/sec3/vgg_v2.png}
    \caption{Effect of first and second split points on VGG16. The vertical axis is the first split point in terms of layers, and the horizontal axis is the second split point counting backwards on layers.}
    \label{vgg_sec3}    
\end{figure}

One of the important findings from \cite{He2019, ding2023patrol}'s study is that increasing the depth (h) of $\mathbf{M}_{c,h}$ will lead to worse image reconstruction quality of the adversarial attacker in MIA. At the same time, part of \cite{Zhou2022ANT}'s algorithm lets the client, instead of the server, compute the Softmax function of $\mathbf{M}(x,\theta)$ at the last layer. The success of their algorithm raises the possibility of utilizing a second split point to enhancing privacy protection. Under the threat model defined by Section 2.2, we provide visual evaluations of the quality of reconstructed images from MIA, as shown by Figure \ref{vgg_sec3} and \ref{res_sec3}. The vertical axis is the position of first split point, and the horizontal axis is the position of second split point counting backwards. For VGG-16 architecture, the first h layers of $\mathbf{M}$ belongs to the client. For the ResNet-18 architecture with 4 blocks, h represents the number of residual blocks computed by the client, with h=1 being the client only computing the first convolutional layer.


\begin{figure}{}
    \centering
    \includegraphics[scale=0.35]{img/sec3/resnet_v2.png}
    \caption{Effect of first and second split points on ResNet-18 with 4 blocks in the shape of [2,2,2,2]. The vertical axis is the first split point, and the horizontal axis is the second counting backwards. When h=1, only the first convolutional layer belongs to the client; when h=2, split point is at the end of the first block; when h=3, the split point is at the second block.}
    \label{res_sec3}
\end{figure}

As shown in the figures, our experiments align with the results from \cite{He2019} and \cite{ding2023patrol}. \textbf{The deeper the first split point is, the worse the reconstructed image is.} However, the experiments do not support the idea from \cite{Zhou2022ANT}. The second split point does not increase the difficulty of reconstruction under MIA. It is also noteworthy to point out that while our experiments indicate that image reconstruction quality is below human-level recognition after h=6 for VGG-16 and h=2 for ResNet-18, this should not be treated as a privacy-guarantee. This is because we are using a standard decoder for $\tilde{\mathbf{M}_{c,h}}(x, \tilde{\theta_{c,h})}$, whereas there exist more powerful generative decoders that could do potentially better at reconstructing images \cite{Khosravy2022GAN}. At the same time, this reconstruction depends on the task. For example, \cite{preva} is able to reconstruct high-quality facial images with larger h, and \cite{ding2023patrol} is more successful with vehicle reconstruction. %We also provide a brief experiment of MIA on NLP task in the Appendix A.1.
